AHEAD: Adaptive Hierarchical Decomposition for Range Query under Local Differential Privacy

For protecting users' private data, local differential privacy (LDP) has been leveraged to provide the privacy-preserving range query, thus supporting further statistical analysis. However, existing LDP-based range query approaches are limited by their properties, i.e., collecting user data according to a pre-defined structure. These static frameworks would incur excessive noise added to the aggregated data especially in the low privacy budget setting. In this work, we propose an Adaptive Hierarchical Decomposition (AHEAD) protocol, which adaptively and dynamically controls the built tree structure, so that the injected noise is well controlled for maintaining high utility. Furthermore, we derive a guideline for properly choosing parameters for AHEAD so that the overall utility can be consistently competitive while rigorously satisfying LDP. Leveraging multiple real and synthetic datasets, we extensively show the effectiveness of AHEAD in both low and high dimensional range query scenarios, as well as its advantages over the state-of-the-art methods. In addition, we provide a series of useful observations for deploying AHEAD in practice.

==> 51_evaluationthree.tex <==
\section{Practical Observations for Deploying \myahead}
\label{Practical Guidelines for Deploying AHEAD}

\label{comprehensive experiment}
In this section, we systematically analyze the impact of user scale, domain size and privacy budget on the performance of \myahead and the state-of-the-art methods. 
When focusing on one variable, we should ensure the others are consistent. 
Therefore, the experiments are mainly conducted on the two synthetic datasets. 
The observations in our following analysis can serve as important guidelines for adopting \myahead in practice 
as well as assessing existing LDP-based range query frameworks. 
\subsection{Impact of User Scale}

\begin{figure*}[!ht]
    \centering
    \subfigure[\myahead, Zipf, Domain size = 256]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/DHIO_MLEApx_CI-Zipf-Domain_8.pdf}
        \label{ahead scale eps zpif}
    }
    \subfigure[\myhio, Zipf, Domain size = 256]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/HIO_Base_CI-Zipf-Domain_8.pdf}
        \label{hio scale eps zpif}
    }
    \subfigure[\mydht, Zipf, Domain size = 256]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/DHT_VP-Zipf-Domain_8.pdf}
        \label{dht scale eps zpif}
    }
    \\[-2ex]
    \subfigure[\myahead, Cauchy, Domain size = 1024]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/DHIO_MLEApx_CI-Cauchy-Domain_10.pdf}
        \label{ahead scale eps cauchy}
    }
    \subfigure[\myhio, Cauchy, Domain size = 1024]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/HIO_Base_CI-Cauchy-Domain_10.pdf}
        \label{hio scale eps cauchy}
    }
    \subfigure[\mydht, Cauchy, Domain size = 1024]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/scale_epsilon/DHT_VP-Cauchy-Domain_10.pdf}
        \label{dht scale eps cauchy}
    }
    \vspace{-0.5cm}
    \caption{The MSE of different methods when varying user scales and privacy budgets. Result are shown in log scale. }
    \vspace{-0.4cm}
    \label{scale and privacy budget}
\end{figure*}

\mypara{Setup}
We compare the algorithms' performance at increasing user scales, \ie, from $10^3$ to $10^7$. 
Under each user scale $N$, we set 8 different privacy budgets. 
As shown in Figure \ref{scale and privacy budget}, we use heatmaps to illustrate the impact of user scale and privacy budget on the MSE. 

In practical use, 
the privacy budget is usually specified by users for satisfying their privacy requirements. 
Then, the aggregator needs to ensure query accuracy under the fixed privacy budget. 
For instance, when privacy budget $\epsilon = 1$, the aggregator desires MSE not higher than $10^{-2}$ to ensure the accuracy of the query results. 
Figure \ref{ahead scale eps zpif} and \ref{ahead scale eps cauchy} show the MSE of \myahead over different coupling of user scale and privacy budget. 
To meet the accuracy demand, the aggregator needs to collect at least $5 \cdot 10^3$ user records with \myahead. 
In comparison, previous works require more user records (more than $10^4$) for satisfying the same level of accuracy. 
For stronger privacy protection, \ie, smaller privacy budget, all methods require more user records. 
Based on the above observations, we summarize the following guideline for selecting a proper user scale. 

\begin{observation}[Necessity of choosing proper user scale]
    \label{Necessity of choosing proper user scale}
    When the privacy protection strength is fixed, \ie, a determined privacy budget $\epsilon$, one needs to use an appropriate user scale to ensure algorithm performance.
\end{observation}
Next, we take a step further to analyze the relation between user scale and privacy budget in order to provide easy guidelines for selecting user scale. 
As shown in Figure \ref{ahead scale eps zpif} and \ref{ahead scale eps cauchy}, \myahead has similar MSEs under different combinations of user scale and privacy budget. 
When user scale $N_1 = 10^6$ and privacy budget $\epsilon_1 = 0.1$, the MSE of \myahead is $10^{-3.0809}$ on the Zipf dataset. 
In addition, \myahead obtains similar MSE ($10^{-3.0563}$) with $N_1 = 10^4$ and $\epsilon_2 = 1$. 
Based on the results in Figures \ref{hio scale eps zpif}, \ref{hio scale eps cauchy}, \ref{dht scale eps zpif} and \ref{dht scale eps cauchy}, \myhio and \mydht also have the user scale \& privacy budget exchangeability. 
All the three evaluated methods leverage the \fo protocol when collecting user private data. 
From Equation \ref{OUEVAR}, 
the variance of \oue is $\frac{4e^{\epsilon}}{N\left(e^{\epsilon}-1\right)^{2}}$. 
The \myvar can be converted to $\frac{4}{N\left(e^{\epsilon}+e^{-\epsilon}-2\right)}$, which is approximate to $\frac{4}{N\epsilon^2}$ when $\epsilon$ is not large ($\epsilon \leq 2$). 
Then, the variance of the estimated frequency is approximately the same if the product $N\epsilon^2$ of two combinations is equal. 
Therefore, we have the following guideline. 
\begin{observation}[The exchangeability between User scale and Privacy budget]
    \label{User scale-Privacy budget exchangeability}
    For any two pairs of user scale and privacy budget combination ($N_1$, $\epsilon_1$) and ($N_2$, $\epsilon_2$), when $\epsilon$ is not large and $N_1\epsilon^2_1 \approx N_2\epsilon^2_2$ is satisfied, \myahead can achieve a similar MSE under two pairs ($N_1$, $\epsilon_1$) and ($N_2$, $\epsilon_2$). 
    \label{Scale-epsilon exchangeability}
\end{observation}
\subsection{Impact of Domain Size}
\label{Impact of Domain Size}

\begin{figure*}[t]
    \centering
    \subfigure[\myahead, Zipf, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/DHIO_MLEApx_CI-Zipf-Set_10_5.pdf}
        \label{ahead domainsize eps zpif}
    }
    \subfigure[\myhio, Zipf, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/HIO_Base_CI-Zipf-Set_10_5.pdf}
        \label{hio domainsize eps zpif}
    }
    \subfigure[\mydht, Zipf, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/DHT_VP-Zipf-Set_10_5.pdf}
        \label{dht domainsize eps zpif}
    }
    \\[-2ex]
    \subfigure[\myahead, Cauchy, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/DHIO_MLEApx_CI-Cauchy-Set_10_5.pdf}
        \label{ahead domainsize eps cauchy}
    }
    \subfigure[\myhio, Cauchy, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/HIO_Base_CI-Cauchy-Set_10_5.pdf}
        \label{hio domainsize eps cauchy}
    }
    \subfigure[\mydht, Cauchy, User scale = $10^5$]{
        \includegraphics[width=0.3\hsize]{./figures_experiment_result/domain_epsilon/DHT_VP-Cauchy-Set_10_5.pdf}
        \label{dht domainsize eps cauchy}
    }
    \vspace{-0.5cm}
    \caption{The MSE of different methods when varying domain sizes and privacy budgets. Result are shown in log scale. }
    \vspace{-0.4cm}
    \label{domainSizeVSPrivacyBudget}
\end{figure*}
\mypara{Setup}
There are 8 different domain sizes 
used in the experiments. 
In addition, we set 7 different privacy budgets 
to explore the coupling effect of domain size $|D|$ and privacy budget $\epsilon$ on MSE. 

1) From Figures \ref{hio domainsize eps zpif}, \ref{dht domainsize eps zpif}, \ref{hio domainsize eps cauchy} and \ref{dht domainsize eps cauchy}, 
the MSEs of \myhio and \mydht have a tendency to increase with the increase of domain size. 
Since all the three algorithms adopt the user partition strategy and the number of groups grows with the domain size, 
the user scale in each group becomes smaller for a larger domain size. 
For example, when domain size rises from $32$ to $4096$, the number of user groups enlarges from 5 to 12 for \mydht. 
Based on Equations \ref{GRRVAR} and \ref{OUEVAR}, the variance of the \fo algorithm is inversely proportional to user scale. 
2) As shown in Figures \ref{ahead domainsize eps zpif} and \ref{ahead domainsize eps cauchy}, \myahead is less affected by the changes in domain size. 
Due to the threshold setting, \myahead makes the actual domain size smaller by amalgamating some lower frequency sub-domains. 
In addition, \myahead averages the estimated frequency values of repeated sub-domains, \eg, sub-domain $[0, 3]$ in Figure \ref{AHEAD method}, to reduce the influence of noise. 
Based on the results in Figure \ref{domainSizeVSPrivacyBudget} and the above analysis, we have the following guideline on the impact of domain size. 

\begin{observation}[Robustness under various domain sizes] 
    \label{Robustness under various domain size}
    The impact of varying domain size on \myahead is different from \myhio and \mydht. \myahead reacts more robust to domain size changes. 
    \vspace{-0.2cm}
\end{observation}

\subsection{Impact of Dataset Skewness}
{\color{red}
\mypara{Setup}
We compare the algorithms' performance at various data skewnesses, where the data records are sampled from low skewness (0 for both \Gaussian and \Laplacian) to high skewness (0.9 for \Gaussian and 2.0 for \Laplacian). 
As shown in \autoref{skewness and privacy budget}, 
under each user scale, we set 8 different privacy budgets and use heatmaps to illustrate the impact of skewness and privacy budget on the MSE. 

1) From \autoref{ahead skewness eps 105 gaussian} and \autoref{ahead skewness eps 105 laplace}, when privacy budget $\epsilon \leq 0.1$, the MSEs of \myahead have a tendency to decrease with the increase of data skewness. 
Since there may exist more nodes suitable for pruning for data with higher skewness, \ie, more sparse sub-domains, \myahead can significantly suppress the injected noises. 
2) With the increase of privacy budget or user scale, the impact of skewness becomes insignificant on MSE of \myahead. 
Recall \autoref{theta setting1} in \autoref{Selection parameters}, the threshold $\theta$ becomes small with large privacy budget or user scale. 
For instance, $\theta = 0.11$ when $\epsilon=0.1$ and $N = 10^6$, and $\theta=0.003$ when $\epsilon=1$ and $N = 10^7$. 
For large privacy budgets or user scales, \myahead reduces the intensity of tree pruning, where the impact of data skewness on the tree construction will be weaken. 

\begin{observation}[The benefit from high skewness]
    \label{The benefit from high skewness}
    \myahead tends to have smaller MSE on highly skew data, where the impact of skewness will weaken as the privacy budget or user scale increases. 
\end{observation}
}

\begin{figure*}[!ht]
    \centering
    \subfigure[\myahead, Gaussian, User scale=$10^5$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Normal_Skew-Set_10_5-Domain_10.pdf}
        \label{ahead skewness eps 105 gaussian}
    }
    \subfigure[\myahead, Gaussian, User scale=$10^6$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Normal_Skew-Set_10_6-Domain_10.pdf}
        \label{ahead skewness eps 106 gaussian}
    }
    \subfigure[\myahead, Gaussian, User scale=$10^7$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Normal_Skew-Set_10_7-Domain_10.pdf}
        \label{ahead skewness eps 107 gaussian}
    }
    \\[-2ex]
    \subfigure[\myahead, Laplacian, User scale=$10^5$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Laplace_Skew-Set_10_5-Domain_10.pdf}
        \label{ahead skewness eps 105 laplace}
    }
    \subfigure[\myahead, Laplacian, User scale=$10^6$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Laplace_Skew-Set_10_6-Domain_10.pdf}
        \label{ahead skewness eps 106 laplace}
    }
    \subfigure[\myahead, Laplacian, User scale=$10^7$]{
        \includegraphics[width=0.31\hsize]{./figures_experiment_result/skewness_epsilon/0329MSE_skewness_ep-Laplace_Skew-Set_10_7-Domain_10.pdf}
        \label{ahead skewness eps 107 laplace}
    }
    \vspace{-0.5cm}
    \caption{The MSE of \myahead when varying dataset skewnesses and privacy budgets. Result are shown in log scale. }
    \vspace{-0.4cm}
    \label{skewness and privacy budget}
\end{figure*}

\subsection{Impact of Attribute Dimension}

{\color{red}
\mypara{Setup}
In this section, we evaluate the performance of \myahead and \myHDG with varying dimensions of data, which are sampled from multivariate \Laplacian and \Gaussian distribution correlation coefficient $r = 0.8$. 

From \autoref{fig: varying attribute dimension}, \myahead is robust to the changes in data dimension. 
Recalling \autoref{Extension to Multi-dimensional Settings}, with the data dimension $m$ increasing, \lle needs to divide users into more groups due to more attribute combinations, \ie, holding fewer user records to estimate the frequency for each 2-dim \myahead tree. 
For instance, when $m = 3$, the number of attribute combination is $C_3^2 = 3$, and when $m = 10$, the number of attribute combination is $C_{10}^2 = 45$. 
Since \lle constructs a query set with associated $2^m$ queries (recall Algorithm \ref{Estimating Answer of m-dimensional Range Query} in \autoref{Extending AHEAD to higher-dimensional range query}), 
the maximum entropy optimization step of \lle incorporates more query information with higher dimension, thus resulting in almost consistent MSEs with dimension increasing. 

\begin{observation}[Robustness under various data dimension] 
    \label{Robustness under various data dimension}
    With the benefit of maximum entropy optimization, the MSE of \myahead is not sensitive to data dimension changes. 
    \vspace{-0.2cm}
\end{observation}
}

\begin{figure*}[!ht]
    \centering
    \subfigure[\Laplacian, $N=10^6$, $|D|= 64^m$]{
    \includegraphics[width=0.235\hsize]{./figures_experiment_result/various_dimension/0416_CI_Rand-Attribute-Ten_Laplace08-Set_10_6.pdf}
    \label{fig: Attribute-Ten_Laplace08-Set_10_6}
    }
    \subfigure[\Laplacian, $N=10^7$, $|D|= 64^m$]{
    \includegraphics[width=0.23\hsize]{./figures_experiment_result/various_dimension/0416_CI_Rand-Attribute-Ten_Laplace08-Set_10_7.pdf}
    \label{fig: Attribute-Ten_Laplace08-Set_10_7}
    }
    \subfigure[\Gaussian, $N=10^6$, $|D|= 64^m$]{
    \includegraphics[width=0.235\hsize]{./figures_experiment_result/various_dimension/0416_CI_Rand-Attribute-Ten_Normal08-Set_10_6.pdf}
    \label{fig: Attribute-Ten_Normal08-Set_10_6}
    }
    \subfigure[\Gaussian, $N=10^7$, $|D|= 64^m$]{
    \includegraphics[width=0.235\hsize]{./figures_experiment_result/various_dimension/0416_CI_Rand-Attribute-Ten_Normal08-Set_10_7.pdf}
    \label{fig: Attribute-Ten_Normal08-Set_10_7}
    }\\[-1ex]
    \subfigure{\includegraphics[width=0.45\textwidth]{./figures_others/comparison_3D_legend3}}  
    \vspace{-0.4cm}
    \caption{The MSE of \myahead when varying attribute dimension $m$ with $\epsilon = 1.1$. Result are shown in log scale. }
    \label{fig: varying attribute dimension}
\end{figure*}

\subsection{Impact of Attribute Correlation}
\label{Impact of Attribute Correlation}
Next, we evaluate the impact of different attribute correlations on query errors as shown in \autoref{3-dim correlation} and \autoref{5-dim correlation}. 
The experimental settings are similar to 2-dim scenes, \ie, varying the correlation coefficient $r$ from 0.1 (\emph{representing weakly correlated}) to 0.9 (\emph{representing strongly correlated}) with a fixed privacy budget $\epsilon = 1.1$. 
From the results, we have the following findings. 
1) The \lle method can protect the correlation between attributes in high-dimensional situations. 
Instead of decomposing all dimensions simultaneously like \de, \lle uses the 2-dim \myahead tree to estimate the answers of high-dimensional range queries. The MSE of \myahead behaves consistently across different correlations, thus the correlation of the data is well preserved by \lle. 
2) The impact of attribute correlation becomes less on \myHDG. 
With the increase of dataset dimension, the number of 1-dim grids ($C_m^2$) increases faster than the 1-dim grids ($C_m^1$). 
Therefore, as shown in \autoref{5-dim correlation}, the negative impact of the 1-dim grids on the correlation is reduced. 

\begin{figure*}[h!]
    \centering
    \subfigure[$N=10^6$, Laplacian, vary $r$]{\label{fig:Three_LaplaceCorr-Set_10_6-Domain_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Three_Laplace-Set_10_6-Domain_6_6_6.pdf}}
    \subfigure[$N=10^7$, Laplacian, vary $r$]{\label{fig:Three_LaplaceCorr-Set_10_7-Domain_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Three_Laplace-Set_10_7-Domain_6_6_6.pdf}}
    \subfigure[$N=10^6$, Gaussian, vary $r$]{\label{fig:Three_NormalCorr-Set_10_6-Domain_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Three_Normal-Set_10_6-Domain_6_6_6.pdf}}
    \subfigure[$N=10^7$, Gaussian, vary $r$]{\label{fig:Three_NormalCorr-Set_10_7-Domain_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Three_Normal-Set_10_7-Domain_6_6_6.pdf}}\\[-1ex]
    \subfigure{\includegraphics[width=0.8\textwidth]{./figures_others/comparison_3D_legend5}}  
    \vspace{-0.4cm}
    \caption{Comparison of different methods on 3-dim \Laplacian and \Gaussian datasets under various attribute correlation. Results are shown in log scale.}
    \vspace{-0.4cm}
    \label{3-dim correlation}
\end{figure*}

\begin{figure*}[h!]
    \centering
    \subfigure[$N=10^6$, Laplacian, vary $r$]{\label{fig:Five_LaplaceCorr-Set_10_6-Domain_6_6_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Five_Laplace-Set_10_6-Domain_6_6_6_6_6.pdf}}
    \subfigure[$N=10^7$, Laplacian, vary $r$]{\label{fig:Five_LaplaceCorr-Set_10_7-Domain_6_6_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Five_Laplace-Set_10_7-Domain_6_6_6_6_6.pdf}}
    \subfigure[$N=10^6$, Gaussian, vary $r$]{\label{fig:Five_NormalCorr-Set_10_6-Domain_6_6_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Five_Normal-Set_10_6-Domain_6_6_6_6_6.pdf}}
    \subfigure[$N=10^7$, Gaussian, vary $r$]{\label{fig:Five_NormalCorr-Set_10_7-Domain_6_6_6_6_6}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0406_CI_Correlation-Five_Normal-Set_10_7-Domain_6_6_6_6_6.pdf}}\\[-1ex]
    \subfigure{\includegraphics[width=0.5\textwidth]{./figures_others/comparison_3D_legend3}}  
    \vspace{-0.5cm}
    \caption{Comparison of different methods on 5-dim \Laplacian and \Gaussian datasets under various attribute correlation. Results are shown in log scale.}
    \vspace{-0.4cm}
    \label{5-dim correlation}
\end{figure*}

\subsection{Remarks}
{\color{red}
The five observations mentioned above reflect the impact of various factors on the performance of \myahead. 
Observations 1 and 2 describe the coupling influence of user scale and privacy budget on algorithm accuracy and demonstrate the transformation relationship between the user scale and privacy budget. 
Observation 3 and 5 demonstrates the advantageous robustness of \myahead under different domain sizes and data dimensions. 
Observation 4 provides an encouraging of practical adoption of \myahead when facing highly skew data. 

In detail, 1) when the privacy protection strength (the privacy budget $\epsilon$) is fixed, according to Observation \ref{Necessity of choosing proper user scale}, 
\myahead obtains more accurate query answers with larger user scales. 
2) If the user scale is insufficient, the aggregator tends to pay the cost, such as compensation fee, 
to trade with users to reduce the strength of privacy protection (increasing the privacy budget $\epsilon$). 
From Observation \ref{User scale-Privacy budget exchangeability}, 
the aggregator can readily calculate the appropriate $\epsilon$ based on the user scale. 
3) For the continuous attribute, 
the aggregator divides the total domain into slots of a fixed length 
and bucketize the records at a suitable granularity for queries 
\cite{wang2019answering,cormode2019answering}. 
Therefore, 
when the domain size is 1024, the bucketize granularity is two times that of the domain size 512. 
From Observation \ref{Robustness under various domain size}, since \myahead is more robust to domain size changes, the aggregator can choose a larger domain size to obtain a higher granularity. 
4) When private data tends to have a high skewness, such as data from income, social networks and Web surfing, practitioners should give priority to \myahead from Observation \ref{The benefit from high skewness}. 
5) From Observation \ref{Robustness under various data dimension},
in practice, \myahead can handle the impact of dimension increasing. 
}

\section{Additional Figures and Table}
\label{Extra Figures and Table}
\autoref{table: the cut rate of leaf node} presents the ratio of the number of leaf nodes of the tree with the threshold to the number of leaf nodes of the original tree without the threshold, where privacy budget $\epsilon$ varies from $0.1$ to $1.5$. 
Figure \ref{fig:the distribution of leaf nodes} presents the distributions of the number of leaves under different $\epsilon$. 
Figure \ref{Appendix: 2-dim overall compare} shows the MSEs of different methods over 2-dim \Laplacian and \Gaussian distributions, 
with various attribute correlations $r = 0.7$, $r = 0.8$ and $r = 0.9$. 

\begin{table*}[!ht]
\centering
\caption{The ratio of \myahead leaf nodes to complete tree leaf nodes under different privacy budgets. 
Each cell contains the number of \myahead leaf nodes and the corresponding ratio. 
Each row represents the values for the same $\epsilon$ setting. }
\begin{tabular}{c c c c c c c c c}
\hline
                            & \textbf{Loan} & \textbf{Financial} & \textbf{BlackFriday} & \textbf{Salaries}  & \textbf{Laplacian} & \textbf{Laplacian} & \textbf{Gaussian} & \textbf{Gaussian} \\ 
\textbf{Origin}                 & 256 (1-dim)   & 512  (1-dim)   & 1024  (1-dim)    & 2048  (1-dim)    & $256^2$ (2-dim)                  & $1024^2$  (2-dim)              & $256^2$  (2-dim)               & $1024^2$  (2-dim)  \\ \hline
$\epsilon = 0.1$            & 26 (10.16\%)       & 37 (7.23\%)      & 9 (0.88\%)        & 10 (0.49\%)         & 70 (1.07\textperthousand)        & 70 (0.07\textperthousand)      & 73 (1.11\textperthousand)        & 67 (0.06\textperthousand)       \\
\rowcolor{mygray}                                                                                               
$\epsilon = 0.3$            & 65 (25.39\%)       & 94 (18.36\%)     & 30 (2.92\%)       & 21 (1.03\%)    & 214 (3.27\textperthousand)       & 193 (0.18\textperthousand)     & 205 (3.13\textperthousand)       & 205 (0.20\textperthousand)       \\ 
$\epsilon = 0.5$            & 99 (38.67\%)       & 148 (28.91\%)    & 67 (6.54\%)       & 29 (1.42\%)    & 370 (5.65\textperthousand)       & 325 (0.31\textperthousand)    & 361 (5.51\textperthousand)       & 298 (0.28\textperthousand)       \\ 
\rowcolor{mygray}                                                                                               
$\epsilon = 0.7$            & 115 (44.92\%)      & 191 (37.30\%)    & 85 (8.30\%)       & 38 (1.86\%)    & 472 (7.20\textperthousand)       & 433 (0.41\textperthousand)    & 448 (6.84\textperthousand)       & 424 (0.40\textperthousand)       \\ 
$\epsilon = 0.9$            & 130 (50.78\%)      & 231 (45.12\%)    & 102 (9.96\%)      & 49 (2.39\%)    & 664 (10.13\textperthousand)      & 556 (0.53\textperthousand)    & 619 (9.45\textperthousand)      & 562  (0.54\textperthousand)       \\ 
\rowcolor{mygray}                                                                                               
$\epsilon = 1.1$            & 142 (55.47\%)      & 267 (52.15\%)    & 137 (13.38\%)     & 68 (3.32\%)    & 760 (11.60\textperthousand)      & 682 (0.65\textperthousand)    & 799 (12.19\textperthousand)     & 712  (0.68\textperthousand)       \\ 
$\epsilon = 1.3$            & 147 (57.42\%)      & 294 (57.42\%)    & 152 (14.84\%)     & 71 (3.47\%)    & 943 (14.39\textperthousand)      & 889 (0.85\textperthousand)    & 958 (14.62\textperthousand)     & 823  (0.78\textperthousand)       \\ 
\rowcolor{mygray}                                                                                               
$\epsilon = 1.5$            & 153 (59.77\%)      & 328 (64.06\%)    & 168 (16.41\%)     & 88 (4.30\%)    & 1150 (17.55\textperthousand)     & 1060 (1.01\textperthousand)    & 1147 (17.50\textperthousand)     & 1027 (0.98\textperthousand)       \\ \hline
\end{tabular}
\label{table: the cut rate of leaf node}
\end{table*}


\begin{figure*}[!t]
    \centering
    \subfigure[$|D|=256$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace08-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0118Rand_ep-Two_Laplace07-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace08-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0118Rand_ep-Two_Laplace07-Set_10_7-Domain_10_10.pdf}}
    \subfigure[$|D|=256$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal08-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0118Rand_ep-Two_Normal07-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal08-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0118Rand_ep-Two_Normal07-Set_10_7-Domain_10_10.pdf}}
    
    \centering{Correlation $r = 0.7$} 
    
    \subfigure[$|D|=256$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace08-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Laplace08-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace08-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Laplace08-Set_10_7-Domain_10_10.pdf}}
    \subfigure[$|D|=256$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal08-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Normal08-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal08-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Normal08-Set_10_7-Domain_10_10.pdf}}
    
    \centering{Correlation $r = 0.8$} 
    
    \subfigure[$|D|=256$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace09-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Laplace09-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Laplacian, vary $\epsilon$]{\label{fig:Two_Laplace09-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Laplace09-Set_10_7-Domain_10_10.pdf}}
    \subfigure[$|D|=256$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal09-Set_10_7-Domain_8_8}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Normal09-Set_10_7-Domain_8_8.pdf}}
    \subfigure[$|D|=1024$, Gaussian, vary $\epsilon$]{\label{fig:Two_Normal09-Set_10_7-Domain_10_10}\includegraphics[width=0.24\hsize]{./figures_experiment_result/overall_result/0111Rand_ep-Two_Normal09-Set_10_7-Domain_10_10.pdf}}

    \centering{Correlation $r = 0.9$} 
    
    \subfigure{\includegraphics[width=0.6\textwidth]{./figures_others/comparison_2D_legend5.pdf}}  \\[-2ex]
    \caption{The MSE of different methods with privacy budget varying from 0.1 to 1.5. Results are shown in log scale.} 
    \label{Appendix: 2-dim overall compare}
\end{figure*}

\begin{figure*}[!ht]
    \centering
    \subfigure[Loan, $N=2260668$, $|D|= 256$]{
    \includegraphics[width=0.235\hsize]{./figures_others/0118leaf_Distribution-Loan-Ori-Domain_2_8-1.5-2-20.pdf}
    }
    \subfigure[Financial, $N=6362620$,  $|D|= 512$]{
    \includegraphics[width=0.23\hsize]{./figures_others/0118leaf_Distribution-Financial-Ori-Domain_2_9-1.5-2-20.pdf}
    }
    \subfigure[BlackFriday, $N=537577$,  $|D|= 1024$]{
    \includegraphics[width=0.235\hsize]{./figures_others/0118leaf_Distribution-BlackFriday-Ori-Domain_2_10-1.5-2-20.pdf}
    }
    \subfigure[Salaries, $N=148654$,  $|D|= 2048$]{
    \includegraphics[width=0.235\hsize]{./figures_others/0118leaf_Distribution-Salaries-Ori-Domain_2_11-1.5-2-20.pdf}
    }
    \caption{The distribution of the number of leaves in the \myahead. 
    The top of each picture shows the true frequency distribution, and the bottom shows the corresponding distribution of the number of leaves with $\epsilon$ varying from 0.1 to 1.5. }
    \label{fig:the distribution of leaf nodes}
\end{figure*}

